Microtopia: Exploring the Impact of Interdisciplinary Projects on Ethnic Minority Female Pupils' Perceptions of Computer Science

This paper presents Microtopia, an interdisciplinary programme designed to broaden participation in computer science (CS) among ethnic minority girls. The programme combined coding with design thinking activities, incorporating Artificial Intelligence (AI), the Internet of Things (IoT), and Robotics as key technologies. Learning activities were formulated around the UN Sustainable Development Goals and the Chinese Five Elements philosophy to support problem-based learning. Pupils were organised into "nations" and engaged in sector-based projects (e.g., healthcare, transportation, fashion, tourism, food, architecture). Using pre- and post-questionnaires, we investigated how socioeconomic and ethnocultural factors influenced pupils' preconceptions of CS, and whether participation in Microtopia shifted their perceptions. Through statistical analysis of the questionnaire data, we identified significant increases in students' confidence, enjoyment, and motivation, particularly when computing was presented as relevant to sustainability and global challenges.

==> Old/0.5Results_Old.tex <==
\section{Results}
\label{Results}
\subsection{Socioeconomic Factors Affecting Preconceptions of CS}
This section addresses RQ1: What socioeconomic factors influence ethnic minority girls' preconceptions of CS? Data were collected on parental employment status, highest level of education attained, number of bedrooms in the household, number of siblings, home ownership, access to a personal bedroom, and car ownership. A composite measure of socioeconomic status (SES) was employed to minimise potential bias by increasing variability in SES scores. The composite SES score was structured such that a higher value indicated a higher socioeconomic status. The classification criteria were adapted from Oakes and Andrade (2017) and participants were categorised into three SES groups: 2−4 as low (N = 36), 5−7 as medium (N = 32), and 8−10 as high (N = 22).

\begin{table}[h!]
\centering
\caption{\textbf{Table N.} Descriptive Statistics of socioeconomic factors to students' preconceptions}
\begin{tabular}{lcccccc}
\hline
 & & N & Percentage & Mean & SD & SE \\
\hline
\multirow{4}{*}{Preconception} 
 & Low SES  & ?? & \%    & 3.94 & 0.87 & 0.04 \\
 & Mid SES  & ?? & \%    & 3.93 & 0.84 & 0.05 \\
 & High SES & ?? & \%    & 3.98 & 0.75 & 0.02 \\
 & Total    & 90 & 100\% & 3.96 & 0.80 & 0.02 \\
\hline
\end{tabular}
\end{table}

From the descriptive statistics (see Table N), it is found that all SES groups value collaboration and teamwork, with high SES students showing the strongest agreement. High SES students (mean=??) are more comfortable being the only girl in a group showing high gender inclusivity. Low agreement across SES groups seeing CS as Male-Dominated, suggesting minimal influence of gender stereotypes in CS. High SES students (mean=??) see CS as relevant to real-world, while low SES students (mean=??) perceive less applicability. Due to uneven group subjects, Kruskal-Wallis tests was used to analyse the students' socioeconomic status to their preconceptions of CS using the questionnaire items in Part III.
\begin{table}[htbp]
\centering
\caption{\textbf{Table N.} Results of Kruskal-Wallis tests of socioeconomic factors to students' preconceptions}
\begin{tabular}{lccc cccc}
\hline
 & \multicolumn{3}{c}{Mean (SD)} & \textit{df} & $X^{2}$ & $p$ & \text{Cohen's \textit{d}} \\
\cline{2-4}
 & Low \\ ($N$=??) & Mid \\ ($N$=??) & High \\ ($N$=??) &  &  &  &  \\
\hline
SES & \textit{5.62 (1.64)} & \textit{5.65 (1.05)} & \textit{5.65 (1.05)} & 75 & -0.09 & .93 & 0.02 \\
\hline
\end{tabular}
\end{table}
The Kruskal-Wallis test (see Table N) was conducted to examine differences in socioeconomic status (SES) across three groups: Low, Mid, and High. The results indicate no significant difference among the groups, $\chi^{2}(75) = -0.09$, $p = 0.93$, suggesting that SES did not significantly vary across the three categories. The mean SES scores for the Low ($M = 5.62$, $SD = 1.64$), Mid ($M = 5.65$, $SD = 1.05$), and High ($M = 5.65$, $SD = 1.05$) groups were similar. Additionally, Cohen’s $d = 0.02$, indicating a negligible effect size. These findings suggest that socioeconomic status did not have a meaningful impact on the measured variable in this study.


\subsection{Ethnocultural Factors Affecting Preconceptions of CS}
\textit{RQ2: Which ethnocultural factors influence girls from ethnic minorities’ preconceptions of CS?}
For this \textit{RQ}, individual analyses were conducted to investigate the differences between ethnic groups. However, the majority ethnic group for data collected were (Asian or British Asian [$N = 68$]). Therefore, we also split the data to investigate the possible differences between the majority ethnic group and the minority ethnic groups (Black [$N = 6$], Mixed [$N = 7$], White [N = 5], and Other [$N = 4$]). Both analyses are presented in this section. 
\\
\\
\textbf{Analysis Approach and Descriptive Statistics}

%As per \textit{RQ1}, a one-way ANOVA was also appropriate for investigating \textit{RQ2}. The data were treated as continuous. The test of normality were violated and we cannot  review the Welsh’s statistic due to unequal groups. As a result, a Kruskal Wallis Test ($H$) was conducted, and a Mann Whitney U test was conducted as follow up tests. 
\textit{RQ2} is analysed in the same way as described for \textit{RQ1}.
Descriptive statistics can be seen in Figure \ref{fig:DSRQ2}.
\\
\\
\textbf{Results For Different Ethnicities and Significant Questions}

There was a significant difference between the groups for “I think boys and girls can be good at CS” ($H_{(4)}  = 10.19$, $p = .04$), “I feel good about working on projects with my team mates” ($H_{(4)} = 12.31$, $p = .02$), “I think it is important for us to work together when we have tasks to do” ($H_{(4)} = 10.83$, $p = .03$), “I like when we all help each other to finish out work” ($H_{(4)} = 17.08$, $p = .002$), “It’s easy for me to talk to my teammates and share my ideas when working on something” ($H_{(4)}  = 9.98$, $p = .041$), “I am ok with doing different jobs in our groups when we need to” ($H_{(4)}= 10.25$, $p = .04$), “I think CS is a boys club” ($H_{(4)} = 9.71$, $p = .046$) and “I do not think I work well in a group” ($H_{(4)} = 13.79$, $p = .008$). A Mann-Whitney U was conducted for the follow up tests and can be seen in Table \ref{Tab:PNEM}. 

\begin{figure}[h!]
    \centering
    \includegraphics[width=1\linewidth]{Figures/Result_Imgs/DSRQ2.png}
    \caption{Descriptive statistics for survey responses across different ethnic groups (Asian or Asian British, Black, Mixed, White, and Other). The responses cover various survey questions, including attitudes toward teamwork, communication, and perceptions of computer science. Bars represent mean scores, with error bars indicating the standard error of the mean (SEM). This visualisation highlights variations in perceptions and experiences across ethnic groups for each survey question.}
    \label{fig:DSRQ2}
\end{figure}

\begin{table}[h!]
\centering
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{|p{4cm}|p{7cm}|p{4cm}|}
\hline
\textbf{Ethnic Group} & \textbf{Survey Question} & \textbf{Mann-Whitney U} \\
\hline
Asian or Asian British vs. Black & I feel good about working with my teammates on projects & $U = 0.107, p = 0.04$ \\
\cline{2-3}
 & I think it’s important for us to work together when we have tasks to do & $U = 92, p = 0.02$ \\
\cline{2-3}
 & I like it when we all help each other to finish our work & $U = 76, p = 0.005$ \\
\hline
Asian or Asian British vs. Mixed & Boys and girls can be good at computer science & $U = 131.50, p = 0.009$ \\
\cline{2-3}
 & I feel good about working with my teammates on projects & $U = 98.5, p = 0.008$ \\
\cline{2-3}
 & I think it’s important to work together on projects & $U = 120.50, p = 0.02$ \\
\cline{2-3}
 & I like it when everyone helps to finish work & $U = 81, p = 0.001$ \\
\cline{2-3}
 & It’s easier to talk to teammates & $U = 98.50, p = 0.007$ \\
\cline{2-3}
 & I’m okay with doing different jobs in groups & $U = 105.50, p = 0.01$ \\
\cline{2-3}
 & CS is a boys’ club & $U = 139, p = 0.01$ \\
\cline{2-3}
 & I do not work well in a group & $U = 123, p = 0.02$ \\
\hline
Black vs Mixed & I’m okay with doing different jobs in groups & $U = 7.5, p = 0.051$ \\
\hline
Black vs White & I do not work well in a group & $U = 2.5, p = 0.017$ \\
\hline
Black vs Other & I do not work well in a group & $U = 0, p = 0.01$ \\
\hline
White vs Mixed & I feel good about collaboration on projects & $U = 4.5, p = 0.03$ \\
\cline{2-3}
 & I’m okay with doing different jobs in groups & $U = 4.5, p = 0.03$ \\
\hline
Mixed vs Other & I do not work well in a group & $U = 2, p = 0.024$ \\
\cline{2-3}
 & I’m okay with doing different jobs in groups & $U = 1.5, p = 0.01$ \\
\cline{2-3}
 & Easy to talk to teammates and share ideas & $U = 3, p = 0.042$ \\
\cline{2-3}
 & I feel good about working with teammates on projects & $U = 3, p = 0.042$ \\
\hline
\end{tabular}%
}
\caption{Mann-Whitney U test results analyzing perceptions of teamwork, collaboration, and inclusivity across different ethnic group comparisons in computer science contexts. Significant differences are highlighted with p-values below 0.05, illustrating how various groups perceive teamwork dynamics, communication, and inclusivity in group settings.}
\label{Tab:PNEM}
\end{table}

The analysis revealed differences in collaboration and group work perceptions between ethnic groups. Asian or Asian British students tended to rate different collaborative questions, like feeling good about working with teammates, thinking teamwork is important, and liking when everyone helps, higher than Black students. 
Compared to the Mixed ethnic group, Asian students held more positive views about boys and girls being equally capable in computer science, as well as their own abilities to work effectively in groups. On the other hand, the Mixed group felt computer science was more of a "boys' club" and that they did not work well in groups compared to the Asian students. Black students were more comfortable taking on different roles in groups than the Mixed group but felt they do not work well in groups compared to White and Other ethnic students. Finally, the White group reported positive collaborative attitudes, while the Other group felt good about working with teammates and being flexible in their group roles. 
\\
\\

\begin{table}[h!]
\centering
\caption{Identity strength and community connectedness by ethnicity. Percentages for subgroups with  $N<10$ should be interpreted with caution as they represent very small numbers.}
\small
\begin{tabular}{lccccc}
\hline
Ethnicity & N & Born UK Yes & High Identity Strength (\%) & High Community Connectedness (\%)\\
\hline
Asian  & $68$ & $50$ & $51.5$ & $36.8$ \\
Black  & $6$  & $3$  & $33.3$ & $33.3$ \\
Mixed  & $7$  & $5$  & $28.6$ & $28.6$ \\
White  & $5$  & $5$  & $60$   & $60$   \\
Other  & $4$  & $3$  & $50$   & $75$   \\
\end{tabular}
\label{tab.EthnicityIdentity}
\end{table}
\textbf{Majority Ethnic Group vs Minority Ethnic Group}

The majority ethnic group was Asian or Asian British and compared to the minority group (White, Black, and Other). The descriptive statistics are presented in Figure \ref{fig:DSREM}. 
The results suggest that the ethnic majority group has a stronger preference for collaborative work, where everyone contributes to a shared goal.% of completing work. 
They also find it easier to talk to teammates, suggesting they feel more comfortable and confident in expressing ideas and participating in group discussions. Finally, while the perception that CS is a boys’ club is marginally significant (showing a trend for significance), this suggests that the ethnic majority group feel that CS is a boys club or is often catered to boys. This could reflect broader societal biases or personal experiences. 

\begin{figure}[h!]
    \centering
    \includegraphics[width=1\linewidth]{Figures/Result_Imgs/DSEM.png}
    \caption{Comparison of descriptive statistics for survey responses between Ethnic Majority and Ethnic Minority groups. The bars represent the mean scores for each group on three survey items: (1) "I think it is important for us to work together when we have tasks to do," (2) "I like it when we all help each other to finish our work," and (3) "It’s easy for me to talk to my teammates and share my ideas when we’re working on something." Error bars indicate the standard error of the mean (SEM).}
    \label{fig:DSREM}
\end{figure}

\begin{table}[h!]
\centering
\begin{tabular}{|p{5.5cm}|p{5.5cm}|}
\hline
\textbf{Survey Question} & \textbf{Mann-Whitney U Results} \\
\hline
I think it is important for us to work together when we have tasks to do & $U = 454.50, p = .003$ \\
\hline
I like it when we all help each other to finish our work. & $U = 932, p < .001$ \\
\hline
It’s easy for me to talk to my teammates and share my ideas when we’re working on something. & $U = 539.50, p = .039$ \\
\hline
I think that a computer science club is a boy’s club. & $U = 601, p = .057$ \\
\hline
\end{tabular}
\caption{Mann-Whitney U test results highlighting perceptions of teamwork, inclusivity, and communication in computer science settings. The table displays statistically significant findings ($p < 0.05$) regarding the importance of collaboration, ease of communication, and shared efforts among teammates, as well as a non-significant trend in perceptions of gender exclusivity in computer science clubs.}
\label{tab:Mann-WhitneR}
\end{table}

\subsection{Perceptions of CS}
\textit{RQ3: To what extent did collaborative interdisciplinary computing projects influence ethnic minority girls’ perceptions of CS?} 
\\
\\
\textbf{Analysis Approach and Descriptive Statistics:}

The data is treated as continuous, and because there were no dropouts from pre- to post-workshop, the comparative groups were equal. This allowed a parametric test to be conducted.  The descriptive statistics can be seen in Figure \ref{fig:DSRQ3}, which shows the responses to the survey questions pre-workshop and post-workshop. The data was treated as ordinal and a Wilcoxon Signed Rank Test was conducted where the perceptions from pre-to-post workshop were evaluated. The results are presented in Table \ref{tab:TTEST}. 

The results suggest significant improvements in confidence and enjoyment. Specifically, students reported greater confidence in using computers post-workshop and found CS more enjoyable and interesting to study. Confidence in their ability to succeed in CS courses and their desire to pursue CS-related careers have also improved. While students were also more likely to feel that anyone could learn CS, they felt that CS is hard and those pursuing it need to be very smart. In sum, these results have highlighted the challenges and perceived intellectual demands of CS.  
\begin{figure}[h!]
    \centering
    \includegraphics[width=1\linewidth]{Figures/Result_Imgs/DSRQ3.png}
    \caption{Descriptive statistics comparing pre-workshop and post-workshop responses to attitudes and perceptions about computer science. The bar graph illustrates changes in confidence, interest, and beliefs regarding computer science, highlighting improvements in enjoyment, confidence, and inclusivity perceptions after the workshop. Error bars represent standard deviations.}
    \label{fig:DSRQ3}
\end{figure}
 
\begin{table}[h!]
\centering
\begin{tabular}{|m{5cm}|m{5cm}|m{3cm}|}
\hline
\textbf{Survey Question Preworkshop} & \textbf{Survey Question Postworkshop} & \textbf{Significance} \\ \hline
I feel confident in my skills when using a computer. & During the tasks, I felt confident when using a computer. & $Z = -5.931$, $p < .001$ \\ \hline
I believe computer science is enjoyable. & During the tasks, I found computer science enjoyable. & $Z = -5.454$, $p < .001$ \\ \hline
I am interested in studying computer science. & During the tasks, I found it interesting to study computer science. & $Z = -5.042$, $p < .001$ \\ \hline
I am confident in my ability to do well in computer science courses. & After doing the tasks, I am feeling confident in my ability to do well in computer science. & $Z = -4.014$, $p < .001$ \\ \hline
I want to have a job someday that involves computers. & After doing the tasks, I want to have a job someday that involves computers. & $Z = -2.073$, $p = .038$ \\ \hline
I believe anyone can learn computer science. & While doing the tasks, I felt that anyone can learn computer science. & $Z = -2.033$, $p = .042$ \\ \hline
I believe that learning computer science is hard. & While doing the tasks, I felt learning computer science is hard. & $Z = -4.376$, $p < .001$ \\ \hline
People who do computer science need to be very smart. & While doing the tasks, I felt that people who do computer science need to be very smart. & $Z = -1.983$, $p = .047$ \\ \hline
\end{tabular}
\caption{Results of Results of a paired samples t-test comparing pre-workshop and post-workshop survey responses on attitudes and perceptions about computer science. Significant changes ($p < 0.05$) are observed in confidence, interest, enjoyment, and beliefs about computer science, indicating positive shifts in participants' attitudes and perceptions after the workshop}
\label{tab:TTEST}
\end{table}

